Memorize to Generalize: on the Necessity of Interpolation in High Dimensional Linear Regression

We examine the necessity of interpolation in overparameterized models, that is, when achieving optimal predictive risk in machine learning problems requires (nearly) interpolating the training data. In particular, we consider simple overparameterized linear regression $y = X \theta + w$ with random design $X \in \mathbb{R}^{n \times d}$ under the proportional asymptotics $d/n \to \gamma \in (1, \infty)$. We precisely characterize how prediction (test) error necessarily scales with training error in this setting. An implication of this characterization is that as the label noise variance $\sigma^2 \to 0$, any estimator that incurs at least $\mathsf{c}\sigma^4$ training error for some constant $\mathsf{c}$ is necessarily suboptimal and will suffer growth in excess prediction error at least linear in the training error. Thus, optimal performance requires fitting training data to substantially higher accuracy than the inherent noise floor of the problem.

==> sections/old-proof-regression.tex <==
\section{Proofs for overparameterized linear model}



%This part is bit sketchy, we need to figure out strong duality in general Hilbert space (or solving the functional minimization problem by other means). Suppose we no longer restrict ourselves to linear estimators but consider the general hypothesis class
%\begin{align}
%	\mathcal{H} = \brc{\est{\theta} = \est{\theta}(X,y) \in \prn{\mathbb{R}^{nd + n} \to \mathbb{R}^d}} \, ,
%\end{align}
%and we also assume Gaussianity for the noise vector $w \sim \normal(0, \sigma^2 I_n)$ and the prior $\theta \sim \normal(0, I_d/d)$. In this case, we consider solving the constrained minimization problem in Eq.~\eqref{eq:not-fitting-problem}, i.e.
%\begin{equation*}
%	\begin{aligned}
%			\min_{\est{\theta} \in \mathcal{H}} & \qquad \pred_X \prn{\est{\theta}} \\
%			\mathrm{s.t.} & \qquad \train_X\prn{\est{\theta}}  \geq \epsilon^2 
%		\end{aligned}
%\end{equation*}
%In this case we have the conditional distribution
%
%and therefore
%\begin{align}
%	\pred_X \prn{\est{\theta}} & = \int \normtwo{\est{\theta}(X,y) - \theta}^2 dP_y dP_{\theta |y} \nonumber \\
%	 & = \int \brc{\normtwo{\est{\theta}(X,y) - (X^\top X + \sigma^2 dI)^{-1}X^\top y}^2 + \sigma^2 \Tr \prn{\prn{X^\top X + \sigma^2 d I}^{-1}}} dP_y \, ,
%\end{align}
%and
%\begin{align}
%	\train_X\prn{\est{\theta}} & = \int \normtwo{X \est{\theta}(X,y) - y}^2 dP_y \, .
%\end{align}
%Consider the Hilbert space for $\mathfrak{H}_y:= \brc{f : \mathbb{R}^n \to \mathbb{R}^d}$ endowed with inner product
%\begin{align*}
%	\langle f, g \rangle_{\mathfrak{H}_y} := \int \langle f(y), g(y) \rangle dP_y,
%\end{align*}
%we can then write the constrained problem as
%\begin{equation*}
%	\begin{aligned}
%			\min_{\est{\theta} \in \mathcal{H}} & \qquad \norm{\est{\theta}(X,y) - (X^\top X + \sigma^2 dI)^{-1}X^\top y}_{\mathfrak{H}_y}^2 +\sigma^2 \Tr \prn{\prn{X^\top X + \sigma^2 d I}^{-1}}  \\
%			\mathrm{s.t.} & \qquad \norm{X \est{\theta}(X,y) - y}_{\mathfrak{H}_y}^2  \geq \epsilon^2 
%		\end{aligned}
%\end{equation*}
%If we have strong duality for this Hilbert space, we can write the optimal condition for $\est{\theta}(X,y)$
%\begin{align*}
%	\est{\theta}(X,y) - (X^\top X + \sigma^2 dI)^{-1}X^\top y - \frac{\rho}{d} \cdot  X^\top \prn{X \est{\theta}(X,y) - y} = 0\, .
%\end{align*}
%For $\rho \geq 0$ we can get
%\begin{align}
%	\est{\theta}(X,y) & = (I - \rho X^\top X/d)^{-1} \prn{(X^\top X + \sigma^2 dI)^{-1} - \rho I/d} X^\top y \, .
%\end{align}
%For the $i$-th eigenvalue $\lambda_i^2$ for $X^\top X$, it has
%\begin{align*}
%	\frac{\frac{1}{\lambda_i^2 + d\sigma^2} - \rho/d}{1 - \rho \lambda_i^2/d} \cdot \lambda_i = \frac{1}{\lambda_i} \cdot \prn{1 - \frac{1 - \frac{\lambda_i^2}{\lambda_i^2 + d\sigma^2}}{1 - \rho \lambda_i^2/d}} = \frac{1}{\lambda_i} \cdot \prn{1 - \frac{\sigma^2}{(1 - \rho \lambda_i^2 / d)(\lambda_i^2/d + \sigma^2)}}\, .
%\end{align*}
%This is exactly the optimal shrinkage we should take in Theorem~\ref{thm:cost-isotropic} when $\rho(\epsilon) > 0$.
 
%We first note that $\pred_X \prn{\est{\theta}}$ and $\train_X\prn{\est{\theta}}$ in the minimization problem in Eq.~\eqref{eq:not-fitting-problem} has the following exact forms.
%
%Suppose $X$ has singular value decomposition such that $X = U \Lambda V^\top$, where $U \in \mathbb{R}^{n \times n}, V \in \mathbb{R}^{d \times n}$ have orthonormal columns and $\Lambda$ is a diagonal matrix with
%\begin{align*}
%	\Lambda = \begin{bmatrix}
%		\lambda_1 & & & \\
%		&\lambda_2 & & \\
%		& & \ddots & \\
%		& & &\lambda_n
%	\end{bmatrix} \, , 
%\end{align*}
%where $\lambda_1 \geq \lambda_2 \geq \cdots \geq \lambda_n \geq 0$. The optimal predictor $\est{\theta}$ for the problem in Eq.~\eqref{eq:not-fitting-problem} can be chosen from a smaller subset of $\mathcal{H}$ by the following lemma.
%
%Applying Lemma~\ref{lem:minimizer-form} allows us to further simplify first the generalization error
%\begin{align}
%	\pred_X\prn{\est{\theta}}&= \frac 1 d \norm{AX-I}_F^2 + \sigma^2 \norm{A}_F^2 \nonumber \\
%	& = \frac 1 d \norm{V \Delta \Lambda V^\top - I}_F^2 + \sigma^2 \norm{\Delta}_F^2 \nonumber \\
%	& \stackrel{\mathrm{(i)}}{=} \frac{1}{d} \prn{d - n + \norm{\Delta \Lambda - I}_F^2} + \sigma^2 \norm{\Delta}_F^2  \nonumber \\
%	&= 1 - \frac{n}{d} + \frac{n}{d} \cdot \frac{1}{n} \sum_{i=1}^n \prn{\lambda_i \delta_i -1}^2 + \sigma^2 \sum_{i=1}^n \delta_i^2 \, , \label{eq:mid-pred}
%\end{align}
%where in (i) it is used that by taking any orthogonal matrix $\begin{bmatrix} V & V^\top \end{bmatrix} \in \mathbb{R}^{d \times d}$, we have
%\begin{align*}
%	\norm{V \Delta \Lambda V^\top - I}_F^2 = \norm{\begin{bmatrix} V & V^\perp \end{bmatrix} \begin{bmatrix} \Delta \Lambda & 0 \\ 0 & 0 \end{bmatrix} \begin{bmatrix} V & V^\perp \end{bmatrix}^\top - I}_F^2 =  \norm{\begin{bmatrix} \Delta \Lambda & 0 \\ 0 & -I \end{bmatrix}}_F^2 = d - n + \norm{\Delta \Lambda - I}_F^2\, .
%\end{align*}
%Similarly we can derive the training error
%\begin{align}
%	\train_X\prn{\est{\theta}}&=\frac{1}{nd} \norm{XAX - X}_F^2 + \frac{\sigma^2}{n} \norm{XA-I}_F^2 \nonumber \\
%	&= \frac{1}{nd} \norm{U \Lambda \Delta \Lambda V^\top - U \Lambda V^\top}_F^2 + \frac{\sigma^2}{n} \norm{U \Lambda \Delta U^\top - I }_F^2 \nonumber \\
%	& = \frac{1}{nd}\norm{\Lambda \Delta \Lambda - \Lambda}_F^2 + \frac{\sigma^2}{n} \norm{\Lambda \Delta - I}_F^2 \nonumber \\
%	& = \frac{1}{n} \sum_{i=1}^n \brk{\frac{1}{d}\prn{\lambda_i^2 \delta_i - \lambda_i}^2 + \sigma^2\prn{\lambda_i \delta_i - 1}^2} \nonumber \\
%	& = \frac{1}{n} \sum_{i=1}^n \prn{\lambda_i^2/d + \sigma^2}\prn{\lambda_i \delta_i - 1}^2 \, . \label{eq:mid-train}
%\end{align}
%Denote by the empirical spectral distribution of $\frac 1 d XX^\top$ by its c.d.f.
%\begin{align*}
%	H_n(s) := \frac 1 n \sum_{i=1}^n \ind_{\lambda_i^2/d \leq s} \, .
%\end{align*}
%and for any $\rho \in [-\infty, \lambda_+^{-1})$ we define
%\begin{align} \label{eq:epsilon-finite-n}
%	\epsilon_n(\rho)^2 = \int \frac{\sigma^4}{(1 - \rho s)^2 \prn{s + \sigma^2}} dH_n(s) \, ,
%\end{align}
%whenever $\rho \cdot \lambda_1^2 / d  <1$. By Bai-Yin law (cf.~Theorem~\ref{thm:BY-law}) we know with probability $1$ that $\lambda_1^2/d \to \lambda_+$ and thus $\epsilon_n(\rho)^2$ will be well-defined for large enough $n$. In particular, we have the following lemma exactly solves the constrained minimization problem~\eqref{eq:not-fitting-problem} when the training error is at least $\epsilon_n(\rho)^2$.
%\begin{lemma} \label{lem:minimum-generalization-error-finite-n}
%	Suppose $\lambda_n > 0$ and $\rho \cdot \lambda_1^2/d < 1$. If $\rho \in [-\infty, 0]$ we have
%	\begin{align}
%		\min_{\est{\theta} \in \mathcal{H}\prn{\epsilon_n(\rho)}} \pred_X\prn{\est{\theta}}= 1 - \frac{n}{d} + \frac{n}{d} \int \frac{\sigma^2}{s+\sigma^2} dH_n(s) \, ,
%	\end{align}
%	where
%	\begin{align}
%		(X^\top X + \sigma^2 d I)^{-1} X^\top y \in \argmin_{\est{\theta} \in \mathcal{H}\prn{\epsilon_n(\rho)}} \pred_X\prn{\est{\theta}} \, .
%	\end{align}
%	For any $\rho \in (0, \lambda_+^{-})$ it holds that
%	\begin{align}
%		\min_{\est{\theta} \in \mathcal{H}\prn{\epsilon_n(\rho)}} \pred_X\prn{\est{\theta}}= 1 - \frac n d + \frac n d \int \prn{  \frac{\rho^2 \sigma^4 s}{\prn{1 - \rho s}^2 \prn{s + \sigma^2}}  + \frac{\sigma^2}{s + \sigma^2}} dH_n(s)  \, .
%	\end{align}
%\end{lemma}
%We defer its proof to Appendix~\ref{proof:minimum-generalization-error-finite-n}. Now we want to apply Lemma~\ref{lem:minimum-generalization-error-finite-n} to obtain the limit
%\begin{align*}
%	\lim_{n \to \infty} \min_{\est{\theta} \in \mathcal{H}\prn{\epsilon}} \pred_X\prn{\est{\theta}} 
%\end{align*}
%for any $\epsilon \geq 0$. By Bai-Yin law in Theorem~\ref{thm:BY-law} we know $\rho \cdot \lambda_1^2/d < 1$ will eventually be satisfied whenever $\rho \in [-\infty, \lambda_+^{-1})$, and by \citet{Yaskov14} we also have for $\lambda_n > 0$ eventually with probability $1$. 
%This allows us to invoke Lemma~\ref{lem:minimum-generalization-error-finite-n} for any $\rho \in [-\infty, \lambda_+^{-1})$ and large enough $n$. 
%
%We return to the main proof of the theorem, let $\rho:=\rho(\epsilon)$ satisfy Eq.~\eqref{eq:rho-epsilon-equation}, and we take $\delta > 0$ such that $\rho + \delta < \lambda_+^{-1}$. By weak convergence of the empirical spectral distribution $\mu_n$ to $\mu$ (cf.~Theorem~\ref{thm:MP-law}) and Eq.~\eqref{eq:epsilon-finite-n} we have
%\begin{align*}
%	\lim_{n \to \infty} \epsilon_n(\rho-\delta)^2 = \int \frac{\sigma^4}{(1 - (\rho - \delta) s)^2 \prn{s + \sigma^2}} dH_n(s) \leq \epsilon^2 \leq \int \frac{\sigma^4}{(1 - (\rho + \delta) s)^2 \prn{s + \sigma^2}} dH_n(s) = \lim_{n \to \infty} \epsilon_n(\rho + \delta)^2 \, .
%\end{align*}
%This then implies for all large enough $n$ we will have $\epsilon_n(\rho - \delta) \leq \epsilon \leq \epsilon_n(\rho +\delta)$ and therefore
%\begin{align*}
%	\mathcal{H}\prn{\epsilon_n(\rho-\delta)} \supset \mathcal{H}\prn{\epsilon} \supset \mathcal{H}\prn{\epsilon_n(\rho+\delta)} \, .
%\end{align*}
%In addition, when $\rho = \rho(\epsilon) < 0$ we can take $\delta$ small enough such that $\rho + \delta < 0$, which implies it holds for all large $n$
%\begin{align*}
%	(X^\top X + \sigma^2 d I)^{-1} X^\top y \in \argmin_{\est{\theta} \in \mathcal{H}(\epsilon)}  \pred_X \prn{\est{\theta}} \, .
%\end{align*}
%Let
%\begin{align*}
%	\phi(\rho,s) = \frac{\rho^2 \sigma^4 s}{\prn{1 - \rho s}^2 \prn{s + \sigma^2}} \ind_{\rho > 0}  + \frac{\sigma^2}{s + \sigma^2} \, ,
%\end{align*}
%and invoke Lemma~\ref{lem:minimum-generalization-error-finite-n}, by weak convergence we have
%\begin{align*}
%	1 - \frac{1}{\gamma} + \frac{1}{\gamma} \int \phi(\rho-\delta, s) dH(s) & = \lim_{n \to \infty} \min_{\est{\theta} \in \mathcal{H}\prn{\epsilon_n(\rho-\delta)}} \pred_X\prn{\est{\theta}} \\
%	& \leq \liminf_{n \to \infty} \min_{\est{\theta} \in \mathcal{H}\prn{\epsilon}} \pred_X\prn{\est{\theta}} \nonumber \\
%	& \leq \limsup_{n \to \infty} \min_{\est{\theta} \in \mathcal{H}\prn{\epsilon}} \pred_X\prn{\est{\theta}}  \nonumber \\
%	& \leq \lim_{n \to \infty} \min_{\est{\theta} \in \mathcal{H}\prn{\epsilon_n(\rho+\delta)}} \pred_X\prn{\est{\theta}} = 1 - \frac{1}{\gamma} + \frac{1}{\gamma} \int \phi(\rho+\delta, s) dH(s) \, .
%\end{align*}
%Take $\delta \to 0$ and by continuity, we conclude that
%\begin{align*}
%	\lim_{n \to \infty} \min_{\est{\theta} \in \mathcal{H}\prn{\epsilon}} \pred_X\prn{\est{\theta}} = 1 - \frac{1}{\gamma} + \frac{1}{\gamma} \int \phi(\rho, s) dH(s) \, .
%\end{align*}
%We conclude the proof with
%\begin{align}
%	\lim_{n \to \infty} \cost_X(\epsilon) & = 	\lim_{n \to \infty} \min_{\est{\theta} \in \mathcal{H}\prn{\epsilon}} \pred_X\prn{\est{\theta}} - 	\lim_{n \to \infty} \min_{\est{\theta} \in \mathcal{H}\prn{0}} \pred_X\prn{\est{\theta}} \nonumber \\
%	& = \frac{1}{\gamma} \int \phi(\rho, s) dH(s) - \frac{1}{\gamma} \int \phi(-\infty, s) dH(s) \nonumber \\
%	& = \ind_{\rho > 0} \cdot \frac{\rho^2}{\gamma}  \int \frac{\sigma^4 s}{(1-\rho s)^2 (s + \sigma^2)} dH(s) \, .
%\end{align}



%\subsection{Proof of Lemma~\ref{lem:minimizer-form}} \label{proof:minimizer-form}
%We first observe that by replacing $A$ with $VV^\top A$ doesn't change the constraint but only reducing the objective function since
%\begin{align*}
%	XA = XVV^\top A\, .
%\end{align*}
%Thus we can always assume $A$'s column space and $X$'s row space are the same. Hence we can always take
%\begin{align*}
%	A = V \Delta U^\top \, ,
%\end{align*}
%We only need to show the optimal point must have $\Delta$ being diagonal. The problem also becomes
%\begin{align*}
%	\mathrm{minimize} & \qquad \frac{1}{d}  \norm{\Delta \Lambda - I}_F^2 + \sigma^2 \norm{\Delta}_F^2 \, , \nonumber \\
%	\mathrm{s.t.} & \qquad \frac{1}{nd}\norm{\Lambda \Delta \Lambda - \Lambda}_F^2 + \frac{\sigma^2}{n} \norm{\Lambda \Delta - I}_F^2 \geq \epsilon^2 \, .
%\end{align*}
%We consider the Lagrangian
%\begin{align*}
%	L(\Delta, \lambda) & =  \frac{1}{d}  \norm{\Delta \Lambda - I}_F^2 + \sigma^2 \norm{\Delta}_F^2 - \lambda \prn{\frac{1}{nd}\norm{\Lambda \Delta \Lambda - \Lambda}_F^2 + \frac{\sigma^2}{n} \norm{\Lambda \Delta - I}_F^2 - \epsilon^2} \, ,
%\end{align*}
%and
%\begin{align*}
%	\nabla_{\Delta} L(\Delta, \lambda) & = \frac{2}{d}\prn{\Delta \Lambda^2 - \Lambda} - \frac{2 \lambda \sigma^2}{n}\prn{\Lambda^2 \Delta - \Lambda}   + 2 \sigma^2 \Delta - \frac{2\lambda}{nd} \prn{\Lambda^2 \Delta \Lambda^2 - \Lambda^3} = 0 \, .
%\end{align*}
%Now for any stationary point $\Delta$, along the line
%\begin{align*}
%	\Delta_t = t \diag(\Delta) + (1-t) \Delta
%\end{align*}
%for $t \in [0,1]$, it always holds that $\nabla_{\Delta} L(\Delta_t, \lambda) = 0$, and therefore combining with strong duality for single constraint quadratic optimization (cf.~\citet[Appendix~B.1]{BoydVa04}), we can assume without loss of generality that $\Delta$ is a diagonal matrix.

%\subsubsection{Proof of Lemma~\ref{lem:minimum-generalization-error-finite-n}} \label{proof:minimum-generalization-error-finite-n}
%Suppose $(\lambda_i^2/d +\sigma^2)(\lambda_i \delta_i - 1)^2 = \epsilon_i^2$ for some $\epsilon_i \geq 0$, substituting into Eq.~\eqref{eq:mid-train} we have
%\begin{align*}
%	\est{\theta} \in \mathcal{H}\prn{\epsilon_n(\rho)} \Longleftrightarrow \frac{1}{n} \sum_{i=1}^n \epsilon_i^2 \geq  \epsilon_n(\rho)^2\, .
%\end{align*}
%By this change of variable we can solve
%\begin{align}
%	\delta_i = \frac{1}{\lambda_i} \prn{1 \pm \frac{\epsilon_i}{\sqrt{\lambda_i^2/d + \sigma^2}}} \, ,
%\end{align}
%to minimize the objective $\pred_X(\est{\theta})$ we can see from Eq.~\eqref{eq:mid-pred}
%\begin{align*}
%	\pred_X\prn{\est{\theta}}&= 1 - \frac{n}{d} + \frac{n}{d} \cdot \frac{1}{n} \sum_{i=1}^n \prn{\lambda_i \delta_i -1}^2 + \sigma^2 \sum_{i=1}^n \delta_i^2 \nonumber \\
%	& = 1 - \frac n d + \frac n d \cdot \frac 1 n \sum_{i=1}^n \frac{\epsilon_i^2}{\lambda_i^2/d + \sigma^2} + \sigma^2 \sum_{i=1}^n \delta_i^2 \nonumber \\
%	& \geq 1 - \frac n d + \frac n d \cdot \frac 1 n \sum_{i=1}^n \frac{\epsilon_i^2}{\lambda_i^2/d + \sigma^2} + \sigma^2 \cdot \frac{n}{d} \cdot \frac{1}{n} \sum_{i=1}^n \frac{1}{\lambda_i^2/d} \cdot \prn{1 - \frac{\epsilon_i}{\sqrt{\lambda_i^2/d + \sigma^2}}}^2 \, ,
%\end{align*}
%where the last inequality becomes equality when taking
%\begin{align*}
%	\delta_i = \frac{1}{\lambda_i} \prn{1 -\frac{\epsilon_i}{\sqrt{\lambda_i^2/d + \sigma^2}}}\, .
%\end{align*}
%Thus we only need to solve the problem
%\begin{equation*}
%	\begin{aligned}
%		\min_{\epsilon \geq 0} & \qquad 1 - \frac n d + \frac n d \cdot \frac 1 n \sum_{i=1}^n \frac{\epsilon_i^2}{\lambda_i^2/d + \sigma^2} + \sigma^2 \cdot \frac{n}{d} \cdot \frac{1}{n} \sum_{i=1}^n \frac{1}{\lambda_i^2/d} \cdot \prn{1 - \frac{\epsilon_i}{\sqrt{\lambda_i^2/d + \sigma^2}}}^2 \\
%		\mathrm{s.t.} & \qquad \frac{1}{n} \sum_{i=1}^n \epsilon_i^2 \geq  \epsilon_n(\rho)^2
%	\end{aligned}
%\end{equation*}
%
%\paragraph{Case I: $\rho \leq 0$.} When $\rho \leq 0$ we show that the minimization problem has the same minimizer as that of the unconstrained one. Regardless of the constraint, note that
%\begin{align*}
%	\pred_X\prn{\est{\theta}} & = 1 - \frac n d + \frac n d \cdot \frac 1 n \sum_{i=1}^n \brc{ \frac{\epsilon_i^2}{\lambda_i^2/d + \sigma^2} +  \frac{\sigma^2}{\lambda_i^2/d} \cdot \prn{1 - \frac{\epsilon_i}{\sqrt{\lambda_i^2/d + \sigma^2}}}^2 } \nonumber \\
%	& = 1 - \frac n d + \frac n d \cdot \frac 1 n \sum_{i=1}^n \brc{ \frac{\epsilon_i^2}{\lambda_i^2/d + \sigma^2} \cdot \prn{1 +  \frac{\sigma^2}{\lambda_i^2/d}} - \frac{2 \sigma^2 \epsilon_i}{\lambda_i^2/d \cdot \sqrt{\lambda_i^2/d +\sigma^2}} + \frac{\sigma^2}{\lambda_i^2/d}} \nonumber \\
%	& = 1 - \frac n d + \frac n d \cdot \frac 1 n \sum_{i=1}^n \brc{ \frac{\epsilon_i^2}{\lambda_i^2/d } - \frac{2 \sigma^2 \epsilon_i}{\lambda_i^2/d \cdot \sqrt{\lambda_i^2/d +\sigma^2}} + \frac{\sigma^2}{\lambda_i^2/d}} \nonumber \\
%	& = 1 - \frac n d + \frac n d \cdot \frac 1 n \sum_{i=1}^n \frac{1}{\lambda_i^2 / d}\brc{ \prn{\epsilon_i - \frac{\sigma^2 }{\sqrt{\lambda_i^2/d +\sigma^2}}}^2 - \frac{\sigma^4}{\lambda_i^2/d + \sigma^2} + \sigma^2} \nonumber \\
%	& \geq 1 - \frac n d + \frac n d \cdot \frac 1 n \sum_{i=1}^n \frac{\sigma^2}{\lambda_i^2 / d}\brc{- \frac{\sigma^2}{\lambda_i^2/d + \sigma^2} + 1} \nonumber \\
%	& = 1 - \frac{n}{d} + \frac{n}{d} \int \frac{\sigma^2}{s+\sigma^2} dH_n(s) \, .
%\end{align*}
%The equality holds when taking $\epsilon_i = \sigma^2/ \sqrt{\lambda_i^2/ d +\sigma^2}$, and in this case
%\begin{align*}
%\frac{1}{n} \sum_{i=1}^n \epsilon_i^2 = \int \frac{\sigma^4}{s + \sigma^2} dH_n(s) \geq \int \frac{\sigma^4}{(1 - \rho s)^2 \prn{s + \sigma^2}} dH_n(s)  = \epsilon_n(\rho)^2\, ,
%\end{align*}
%the constraint is satisfied. Further in this case we can write
%\begin{align*}
%	\delta_i = \frac{1}{\lambda_i} \prn{1 - \frac{\sigma^2}{\lambda_i^2/ d +\sigma^2}} = \frac{\lambda_i}{\lambda_i^2 +d\sigma^2},
%\end{align*}
%and hence the optimal $A(X) = V \Delta U^\top$ can then be taken as
%\begin{align*}
%	A(X) = V (\Lambda^2 + d\sigma^2)^{-1} \Lambda  U^\top = \prn{X^\top X + d\sigma^2}^{-1}X^\top \, .
%\end{align*}
%\paragraph{Case II: $\rho > 0$.} We consider the Lagrange dual
%\begin{align*}
%	L(\epsilon, \lambda) & = 1 - \frac n d + \frac n d \cdot \frac 1 n \sum_{i=1}^n \frac{\epsilon_i^2}{\lambda_i^2/d + \sigma^2} + \sigma^2 \cdot \frac{n}{d} \cdot \frac{1}{n} \sum_{i=1}^n \frac{1}{\lambda_i^2/d} \cdot \prn{1 - \frac{\epsilon_i}{\sqrt{\lambda_i^2/d + \sigma^2}}}^2- \lambda \prn{\frac{1}{n} \sum_{i=1}^n \epsilon_i^2 -  \epsilon_n(\rho)^2} \nonumber \\
%	& = 1 - \frac n d + \frac n d \cdot \frac 1 n \sum_{i=1}^n \frac{1}{\lambda_i^2 / d}\brc{ \prn{\epsilon_i - \frac{\sigma^2 }{\sqrt{\lambda_i^2/d +\sigma^2}}}^2 - \frac{\sigma^4}{\lambda_i^2/d + \sigma^2} + \sigma^2} - \lambda \prn{\frac{1}{n} \sum_{i=1}^n \epsilon_i^2 -  \epsilon_n(\rho)^2} \, ,
%\end{align*}
%and it is clearly seen that when $\lambda \geq \lambda_1^2 / d$ we have $\inf_{\epsilon} L(\epsilon, \lambda) = - \infty$. For any $\lambda \in [0, n / \lambda_1^2)$ the minimizer satisfies the stationary condition
%\begin{align*}
%	\nabla_{\epsilon} L(\epsilon, \lambda) = 0 \Rightarrow \frac{n}{d} \cdot \frac{1}{\lambda_i^2/d} \cdot \prn{ \epsilon_i - \frac{\sigma^2}{\sqrt{\lambda_i^2/d + \sigma^2}}} = \lambda \epsilon_i \, .
%\end{align*}
%By strong duality for single quadratic constrained quadratic programming, we obtain the optimality conditions
%\begin{align*}
%	\epsilon_i &= \frac{\sigma^2}{\prn{1 - \frac{n}{d} \lambda \cdot \lambda_i^2/d} \sqrt{\lambda_i^2/d + \sigma^2}} \, , \\
%	\frac{1}{n} \sum_{i=1}^n \epsilon_i^2 & = \epsilon_n(\rho)^2 \, .
%\end{align*}
%Combining these two equations we have
%\begin{align*}
%	\frac{1}{n} \sum_{i=1}^n \epsilon_i^2 & = \frac 1 n \sum_{i=1}^n \frac{\sigma^4}{\prn{1 - \frac{n}{d} \lambda \cdot \lambda_i^2/d}^2 \prn{\lambda_i^2/d + \sigma^2}} = \int \frac{\sigma^4}{\prn{1 - \frac n d \lambda s }^2(s + \sigma^2)} dH_n(s) = \epsilon_n(\rho)^2.
%\end{align*}
%Recall that
%\begin{align*}
%	\epsilon_n(\rho)^2 = \int \frac{\sigma^4}{(1 - \rho s)^2 \prn{s + \sigma^2}} dH_n(s) \, ,
%\end{align*}
%and note that $\epsilon_n(\rho)^2$ is increasing in $\rho \in [-\infty, d/\lambda_1^2)$, we can solve the optimal Lagrange multiplier $\lambda^\star = \frac d n \rho$. Substituting into the objective we get
%\begin{align*}
%	& \min_{\est{\theta} \in \mathcal{H}\prn{\epsilon_n(\rho)}} \pred_X\prn{\est{\theta}} \nonumber \\
%	& = 1 - \frac n d + \frac n d \cdot \frac 1 n \sum_{i=1}^n \frac{1}{\lambda_i^2 / d}\brc{ \prn{ \frac{\sigma^2}{\prn{1 - \rho} \sqrt{\lambda_i^2/d + \sigma^2}} - \frac{\sigma^2 }{\sqrt{\lambda_i^2/d +\sigma^2}}}^2 - \frac{\sigma^4}{\lambda_i^2/d + \sigma^2} + \sigma^2} \nonumber \\
%	& = 1 - \frac n d + \frac n d \int \frac{1}{s} \cdot \brc{ \prn{ \frac{\sigma^2}{\prn{1 - \rho s} \sqrt{s + \sigma^2}} - \frac{\sigma^2 }{\sqrt{s +\sigma^2}}}^2 - \frac{\sigma^4}{s + \sigma^2} + \sigma^2} dH_n(s) \nonumber \\
%	& = 1 - \frac n d + \frac n d \int \frac{1}{s} \cdot \brc{  \frac{\rho^2 \sigma^4 s^2}{\prn{1 - \rho s}^2 \prn{s + \sigma^2}}  + \frac{s\sigma^2}{s + \sigma^2}} dH_n(s) \nonumber \\
%	& = 1 - \frac n d + \frac n d \int \prn{  \frac{\rho^2 \sigma^4 s}{\prn{1 - \rho s}^2 \prn{s + \sigma^2}}  + \frac{\sigma^2}{s + \sigma^2}} dH_n(s) \, .
%\end{align*}
%
%\subsubsection{Proof of Corollary~\ref{cor:threshold-growth}} \label{proof:threshold-growth}
%We first compute the not fitting threshold by taking $\rho = 0$ into Eq.~\eqref{eq:rho-epsilon-equation} and
%\begin{align*}
%	\epsilon_\sigma^2 & = \int \frac{\sigma^4}{s +\sigma^2} dH(s) = \sigma^4 \cdot \lim_{y \to 0^+} S_\gamma(-\sigma^2 + i y) \, ,
%\end{align*}
%where $S_\gamma(z) : \mathbb{C}_+ \to \mathbb{C}_+$, $\mathbb{C}_+ := \brc{z \in \mathbb{C} | z= x+ iy, y > 0}$ is the Stieltjes transformation of the Marchenko-Pastur law, namely
%\begin{align}
%	S_\gamma(z) & = \int \frac{1}{s -z} dH(s) \, .
%\end{align}
%By \citet[Lemma~3.11]{BaiSi10} we can exactly compute
%\begin{align}
%	\epsilon_\sigma^2 & = \sigma^4 \cdot \frac{1 - 1/\gamma + \sigma^2 - \sqrt{\prn{1 + 1 / \gamma + \sigma^2 }^2 - 4/\gamma}}{- 2 \sigma^2/\gamma} \nonumber \\
%	& = \sigma^4 \cdot \frac{ \sqrt{\prn{1 - 1 / \gamma + \sigma^2 }^2 + 4 \sigma^2/\gamma} - \prn{1 - 1 / \gamma + \sigma^2 }}{2 \sigma^2/\gamma} \nonumber \\
%	& = \sigma^4 \cdot \frac{2\sigma^2 / \gamma + o(\sigma^2/\gamma)}{2 \sigma^2/\gamma \cdot \prn{1 - 1/\gamma + \sigma^2}} \nonumber \\
%	& = \frac{\sigma^4}{\sigma^2 + 1 - 1/\gamma} + o(\sigma^4) \, .
%\end{align}


==> sections/preliminaries.tex <==
\section{Preliminaries}

\subsection{Notation}
We denote by $\real$ the set of real numbers and $\mathbb{C}$ the set of complex numbers. We use $\normtwo{u}$ to denote the $\ell_2$ norm of a vector $u$. We also use 
$\norm{M}$ and $\norm{M}_F$ to denote the operator norm and Frobenius norm of a matrix 
$M$. For two vectors $u,v$ of the same dimension, we write $u\geq v$ or $u \leq v$ to
represent entrywise inequality. For two symmetric square matrices $A,B$ of the same dimension we write $A \succ B$ or $A \prec B$ if $A-B$ or $B-A$ is positive definite; we also write $A \succeq B$ or $A \preceq B$ if $A-B$ or $B-A$ is positive semidefinite. For any positive integer $n$, we represent by $[n] := \left\{1, 2, \cdots, n\right\}$. The notation $f(x) = o(g(x))$ for functions $f(x), g(x)$ defined in the neighborhood of $0$ implies $\lim_{x \to 0} f(x)/g(x) = 0$.

For random variables $\xi$ and $\xi_1, \xi_2, \cdots, \xi_n, \cdots$ 
defined on the same probability space with probability distributions $\mu$ and $\mu_1, \mu_2, \cdots, \mu_n, \cdots$, we denote convergence almost surely and 
weakly by $\xi_n \stackrel{a.s.}\to \xi$ and
$\xi_n \Rightarrow \xi$ respectively. We also write $\mu_n \cas \mu$ and $\mu_n \Rightarrow \mu$.

\subsection{Asymptotics of random matrices}

In this section, we review some classical results regarding singular values of random matrices. Consider a triangular array of independent and identically distributed random variables $(z_{ij}(n))_{i\in[n], j\in[d]}$ for $n=1,2,\cdots$ and $d:=d(n)$. We write $Z := Z(n)= (z_{ij}(n)) \in \mathbb{R}^{n \times d}$. Under the proportional asymptotics $d/n \to \gamma \in (0, \infty)$, we have the following standard results of Marchenko-Pastur law and Bai-Yin law.

\begin{lemma}[Marchenko-Pastur law, \citet{BaiSi10}, Thm.~3.4]  \label{thm:MP-law}
	Assume $\mathbb{E}[z_{ij}]=0$ and $\mathbb{E}[z_{ij}^2] = 1$, and suppose $Z$ have singular values $\lambda_1 \geq \lambda_2 \geq \cdots \geq \lambda_n$. Denote the empirical spectral distribution of $\frac 1 d ZZ^\top$ by $\mu_n$ with c.d.f.
\begin{align*}
	H_n(s) := \frac 1 n \sum_{i=1}^n \ind_{\lambda_i^2/d \leq s} \, ,
\end{align*}
then with probability one, $\mu_n \Rightarrow \mu$ where $\mu$ has c.d.f. $H(s)$ and density function
\begin{align} \label{eq:MP-distribution}
	dH(s) = \frac{\gamma}{2\pi} \frac{\sqrt{(\lambda_+ -s)(s - \lambda_-)}}{s} \ind_{s \in [\lambda_-, \lambda_+]} ds \, ,
\end{align}
where $\lambda_{\pm} = \prn{1 \pm 1/\sqrt{\gamma}}^2$.

\end{lemma}

\begin{lemma}[Bai-Yin law, \citet{BaiSi10}, Thm.~5.10]  \label{thm:BY-law}
	Under the same assumptions and notations in Lemma~\ref{thm:MP-law}, the largest singular value $\lambda_1$ and the smallest singular value $\lambda_n$ of $X$ satisfy
	\begin{align}
		\frac{\lambda_1^2}{d} \cas \lambda_+ = \prn{1 + \frac{1}{\sqrt \gamma}}^2 \, , \qquad \frac{\lambda_n^2}{d} \cas \lambda_- = \prn{1 - \frac{1}{\sqrt \gamma}}^2 \, .
	\end{align}
\end{lemma}

Further, we assume there is a deterministic sequence of symmetric positive definite matrices $\Sigma := \Sigma(n) \in \real^{d \times d}$. The following result describes the limit of the empirical spectral distribution of $\frac 1 d Z \Sigma Z^\top$.

\begin{lemma}[Deformed Marchenko-Pastur law, \cite{Silverstein95}]  \label{thm:MP-deformed-law}
	Under the same assumptions in Lemma~\ref{thm:MP-law}, in addition we assume $\Sigma$ has eigenvalues $t_1 \geq t_2 \geq \cdots \geq t_d \geq 0$. Denote the empirical spectral distribution of $\Sigma$ by $\nu_n$ with c.d.f.
	\begin{align*}
		T_n(s) := \frac 1 d \sum_{i=1}^d \ind_{t_i \leq s} \, ,
	\end{align*}
	and suppose $\nu_n$ converges weakly to $\nu$ with c.d.f. $T(s)$. Suppose $Z \Sigma^{\frac 1 2}$ have singular values $\lambda_1 \geq \lambda_2 \geq \cdots \geq \lambda_n$. Denote the empirical spectral distribution of $\frac 1 d Z \Sigma Z^\top$ by $\mu_n$ with c.d.f.
\begin{align*}
		G_n(s) := \frac 1 n \sum_{i=1}^n \ind_{\lambda_i^2/d \leq s} \, ,
\end{align*}
then with probability one, $\mu_n$ converges weakly to $\mu$ with c.d.f. $G(s)$ determined by its Stieltjes transform $m_G : \mathbb{C}_+ \to \mathbb{C}_+$, $\mathbb{C}_+ := \brc{z \in \mathbb{C} | z= x+ iy, y > 0}$ satisfying the fixed point equation
\begin{align}
	m_G(z) = - \prn{z - \int \frac{\tau d T(\tau)}{1 + \tau m_G(z)/\gamma}}^{-1} \, ,
\end{align}
where the Stieltjes transform of a measure on $\real$ with c.d.f. $F$ is defined by
\begin{align}  \label{eq:stieltjes-transform}
	m_F(z) & := \int \frac{1}{s -z} dF(s) \, .
\end{align}
\end{lemma}

\begin{remark}
	The result in Lemma~\ref{thm:MP-deformed-law} is slightly different from that in~\cite[Thm.~1.1]{Silverstein95}, where the original theorem is stated for the empirical spectral distributions of $\frac 1 n Z \Sigma Z^\top$. By a simple change of variables we can obtain Lemma~\ref{thm:MP-deformed-law} and we omit the details.
\end{remark}


==> sections/proof-auxiliary.tex <==
\section{Proofs for overparameterized classification}



